Spatial variation in the basic reproduction number of COVID-19: A systematic review

OBJECTIVES: Estimates of the basic reproduction number (R0) of COVID-19 vary across countries. This paper aims to characterise the spatial variability in R0 across the first six months of the global COVID-19 outbreak, and to explore social factors that impact R0 estimates at national and regional level. METHODS: We searched PubMed, LitCOVID and the WHO COVID-19 database from January to June 2020. Peer-reviewed English-language papers were included that provided R0 estimates. For each study, the value of the estimate, country under study and publication month were extracted. The median R0 value was calculated per country, and the median and variance were calculated per region. For each country with an R0 estimate, the Human Development Index (HDI), Sustainable Mobility Index (SMI), median age, population density and development status were obtained from external sources. RESULTS: A total of 81 studies were included in the analysis. These studies provided at least one estimate of R0, along with sufficient methodology to explain how the value was calculated. Values of R0 ranged between 0.48 and 14.8, and between 0.48 and 6.7 when excluding outliers. CONCLUSIONS: This systematic review provides a comprehensive overview of the estimates of the basic reproduction number of COVID-19 globally and highlights the spatial heterogeneity in R0. Higher values were recorded in more developed countries, and countries with an older population or more sustainable mobility. Countries with higher population density had lower R0 estimates. For most regions, variability in R0 spiked initially before reducing and stabilising as more estimates became available.

==> FiguresAndTables.tex <==
\begin{document}

\begin{figure}
    \centering
    \includegraphics[width = 8cm]{Images/PRISMA.pdf}
    \caption{Article  screening and data extraction process for the systematic review \cite{moher2009} }
    \label{fig:PRISMA}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.35]{Images/WorldMapSmall.png}
	\end{center}
	\caption{Countries included in the study. \label{fig:WorldMap}}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.6]{Images/hist4.png}
	\end{center}
	\caption{Distribution of $R_0$ values by publication month. \label{fig:Histogram}}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.35]{Images/MediansSmall.png}
	\end{center}
	\caption{National $R_0$ medians as of June 2020. \label{fig:NationalMedians}}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.35]{Images/RegionMediansSmall.png}
	\end{center}
	\caption{Regional $R_0$ medians as of June 2020. \label{fig:RegionalMedians}}
\end{figure}

\begin{figure}
	\begin{center}
		\includegraphics[scale=0.35]{Images/MedianPlotLarge.png}
	\end{center}
	\caption{Region medians over time. The bands show 10\% of the standard deviation. \label{fig:MedianPlot}}
\end{figure}

\begin{figure}
	\begin{center}
		\begin{tabular}{cc}
			\includegraphics[scale=0.3]{Images/HDIPlotLarge.png} &
			\includegraphics[scale=0.3]{Images/AgePlotLarge.png} \\
			a) & b) \\
			\includegraphics[scale=0.3]{Images/SMIPlotLarge.png} &
			\includegraphics[scale=0.3]{Images/PopDensPlotLarge.png}\\
			c) & d)
		\end{tabular}
		\caption{Relationship of $R_0$ to social factors. a) Median $R_0$ by HDI. Points are grouped according to developed-or-transitioning or developing economies. b) Median $R_0$ by median age. Points are grouped according to countries with a median age of 30 and over, or below 30. c) Median $R_0$ by SMI. d) Population density. For the purpose of the visualisation, countries with population density above 12 000 were excluded, namely Bangladesh, Singapore and Hong Kong.}
		\label{fig:Scatterplots}
	\end{center}
\end{figure}

\begin{table}
	\begin{center}
		\caption{Estimates of $R_0$ in South Africa \cite{nicd2020}. \label{tab:NICDR0}}
		\begin{tabular}{p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}p{1.5cm}} 
			Region & South Africa & Western Cape & Gauteng & Eastern Cape & KwaZulu-Natal \\ 
            $R_0$ estimate & 2.07 & 1.76 & 2.19 & 1.84 & 1.73 \\ 
            95\% CI & (1.69, 2.5) & (1.11, 2.62) & (1.95, 2.39) & (1.1, 2.84) & (1.15, 2.47)
        	\tabularnewline 
		\end{tabular}
	\end{center}
\end{table}

[Raeesa's figure.]

\end{document}
